DevMuT: Testing Deep Learning Framework via Developer Expertise-Based Mutation

Deep learning (DL) frameworks are the fundamental infrastructure for various DL applications. Framework defects can profoundly cause disastrous accidents, thus requiring sufficient detection. In previous studies, researchers adopt DL models as test inputs combined with mutation to generate more diverse models. Though these studies demonstrate promising results, most detected defects are considered trivial (i.e., either treated as edge cases or ignored by the developers). To identify important bugs that matter to developers, we propose a novel DL framework testing method DevMuT, which generates models by adopting mutation operators and constraints derived from developer expertise. DevMuT simulates developers'common operations in development and detects more diverse defects within more stages of the DL model lifecycle (e.g., model training and inference). We evaluate the performance of DevMuT on three widely used DL frameworks (i.e., PyTorch, JAX, and Mind- Spore) with 29 DL models from nine types of industry tasks. The experiment results show that DevMuT outperforms state-of-the-art baselines: it can achieve at least 71.68% improvement on average in the diversity of generated models and 28.20% improvement on average in the legal rates of generated models. Moreover, DevMuT detects 117 defects, 63 of which are confirmed, 24 are fixed, and eight are of high value confirmed by developers. Finally, DevMuT has been deployed in the MindSpore community since December 2023. These demonstrate the effectiveness of DevMuT in detecting defects that are close to the real scenes and are of concern to developers.

==> chapters/6_relatedwork.tex <==
% \section{Related work}
% \label{sec:relatwork}

% % \subsection{Model-Level Framework Testing Methods}
% Researchers often adopt DL models as test inputs for DL frameworks: they first generate DL models across multiple DL frameworks and then analyze the results with the same input data.
% Existing work can be divided into two types: (1) some researchers utilize mutation operators to modify existing DL models in public repositories~\cite{pham2019cradle,guo2020audee,wang2020lemon,li2023comet}; (2) some researchers generate new models based on predefined templates and constraint rules~\cite{gu2022muffin,liu2023neuri,liu2023generation,luo2021graphfuzz,wang2022eagle}. The detailed introduction is as follows.

% \subsection{Mutation-Based Testing Methods} 
% Hung Pham et al.~\cite{pham2019cradle} proposed CRADLE, the first model-level testing method that utilizes differential testing by analyzing model execution on different backends of Keras~\cite{keras} (e.g., TensorFlow~\cite{tensorflow}, CNTK~\cite{cntk}). 
% Wang et al.~\cite{wang2020lemon} proposed LEMOM and adopted mutation operators in DeepMutation~\cite{ma2018deepmutation} and DeepMutation++~\cite{hu2019deepmutation++} combined with the MCMC strategy, which has been widely used in many fields~\cite{chen2015guided,Chen2016Coverage2} to guide the mutation generation process. Finally, LEMON utilizes differential testing on the generated mutants to detect defects. 
% Guo et al.~\cite{guo2020audee} proposed Audee, which combined genetic evolution~\cite{vidnerova2016evolutionary} strategy with input-mutation to generate new models that can trigger higher inconsistency and outlier output. 
% Li et al.~\cite{li2023comet} proposed COMET and added new types of mutation operators, such as parameter-mutation and outlier mutation, compared with LEMON. Its execution process is similar to LEMON.


% \subsection{Generation-Based Testing Methods} 
% Gu et al.~\cite{gu2022muffin} proposed Muffin, which generates new models based on the structure of the directed acyclic graph. It focuses on detecting inconsistency defects in three model execution processes: forward propagation, loss calculation, and backward calculation. 
% Wang et al.~\cite{wang2022eagle} proposed EAGLE, which generates models based on these equivalent rules and detects defects by analyzing the consistency of execution results between the original and the equivalent model.
% Luo et al.~\cite{luo2021graphfuzz} proposed Graphfuzz to test DL inference engines based on graph theory. It combines six mutation operators with the MCTS algorithm~\cite{Coulom2006EfficientSA} to explore the generation of new model structures. 
% Liu et al.~\cite{liu2023generation} proposed Gandalf, which generates different models using context-free syntax combined with the DQN~\cite{mnih2015human}. It introduces 15 metamorphic relationships to enhance the testing effectiveness of different DL frameworks. 
% Liu et al.~\cite{liu2023neuri} proposed Neuri, which generates models through inductive rules. It first collects the call relationships of framework interfaces from external resources and analyzes legal interface groups to generate test inputs that can explore the deeper execution behavior of DL frameworks.



% \noindent\textbf{Comparison with Previous Studies.} DevMuT belongs to the mutation-based testing methods and has the following differences compared with existing methods:
% \textbf{Mutation Operators.} The mutation operators adopted in existing methods are directly from the DL model testing work~\cite{ma2018deepmutation,hu2019deepmutation++,humbatova2021deepcrime} while the mutation operators in DevMuT are abstracted from the common experience of developers on DL models.
% \textbf{Mutation Constraints.} Existing work will filter those crash models while DevMuT will further filter those far away from real scenes.
% \textbf{Detection Scope.} Existing work focuses on detecting the defects exposed in model inference while DevMuT detects defects from more stages of the lifecycles of DL models like training.\looseness=-1


% \subsection{API-Level Framework Testing Methods}
% DL frameworks encapsulate a large number of complex functionalities into operators for users. Therefore, researchers also conduct studies on testing these framework interfaces. Among them, some researchers conduct separate analyses on the framework interface by investigating their parameter settings and inputs under constraint conditions. 
% Wei et al.~\cite{Wei2022FreeLF} propose Freefuzz, which mines the input of the framework interface from technical communities and wild code fragments. Then, it mutates the collected original input and tests the target framework interface. 
% Xie et al.~\cite{Xie2021LeveragingDT} propose D2C, another fuzz testing tool that extracts interface constraints from document descriptions to guide the generation of large amounts of testing data and detect defects in the interface.

% Besides, some researchers detect interface defects by analyzing the correlation between framework interfaces. 
% Deng et al.~\cite{Deng2022FuzzingDL} test those framework interfaces with high input/output parameter similarity by automatically inferring their relationships based on the semantics and then analyzing the consistency of the execution state of interfaces. 
% Yang et al.~\cite{Yang2023FuzzingAD} focus on testing those interfaces related to automatic differential calculation. They abstract such interfaces as the functions for processing tensors and then compare the accuracy of their gradient calculation results to detect potential defects. 
% Zhang et al.~\cite{zhang2021predoo} propose Predoo, a DL operator accuracy testing method, which mutates the test input of DL operators to extend the numerical accuracy to maximize the detection of accuracy errors in deep learning frameworks.

% With the rapid development of large language models (LLM), researchers also have attempted to apply LLMs in framework testing~\cite{deng2023large1, deng2023large2}. Deng et al.~\cite{deng2023large1} propose the first LLM-based testing method, TitanFuzz. It produces the test cases and then mutates them based on the generative-style and infill-style prompts to LLMs, respectively. Lately, they find that TitanFuzz tends to generate test cases that are already existing and cannot explore newer state space. To solve this, Deng et al.~\cite{deng2023large2} subsequently proposed FuzzGPT, which adopts prompt or fine-tuning to make LLMs learn from historical test inputs automatically.







